Using wavelets to capture deviations from smoothness in galaxy-scale strong lenses

Modeling the mass distribution of galaxy-scale strong gravitational lenses is a task of increasing difficulty. The high-resolution and depth of imaging data now available render simple analytical forms ineffective at capturing lens structures spanning a large range in spatial scale, mass scale, and morphology. In this work, we address the problem with a novel multiscale method based on wavelets. We tested our method on simulated Hubble Space Telescope (HST) imaging data of strong lenses containing the following different types of mass substructures making them deviate from smooth models: (1) a localized small dark matter subhalo, (2) a Gaussian random field (GRF) that mimics a nonlocalized population of subhalos along the line of sight, and (3) galaxy-scale multipoles that break elliptical symmetry. We show that wavelets are able to recover all of these structures accurately. This is made technically possible by using gradient-informed optimization based on automatic differentiation over thousands of parameters, which also allow us to sample the posterior distributions of all model parameters simultaneously. By construction, our method merges the two main modeling paradigms - analytical and pixelated - with machine-learning optimization techniques into a single modular framework. It is also well-suited for the fast modeling of large samples of lenses. All methods presented here are publicly available in our new Herculens package.

==> Herculens - Wavelets in the potential with autodiff/inferred_perturbations.tex <==
\begin{table*}[!tbh]
\caption{Recovered properties of potential perturbations, from the MAP \lenspotpix models shown on Fig.~\ref{fig:model_summary_pix_pot_real}. The quoted values for the subhalo mass is given in solar units and computed within the region with S/N(\lenspotpix) > 3 (see Fig.~\ref{fig:subhalo_position_mass} and text for more details). The input GRF parameters are given with uncertainties as they were fitted on the power-spectrum of the input perturbing field.}
\label{tab:param_estimations}
\renewcommand{\arraystretch}{1.8}
\centering
\small{
\begin{tabular}{lcclc}
Lens & Parameters & Input values & Model & Measured values \\
\hline
\hline
\multirow{4}*{LS} & \multirow{2}*{$\big(\theta_{x,\rm sub},\theta_{y,\rm sub}\big)$} & \multirow{2}*{$\big( 1.90, -0.40 \big)$} & pixelated & $\big( 1.94 \pm 0.12, -0.49 \pm 0.12 \big)$ \\
 & & & refined & $\big( 1.899 \pm 0.008, -0.408 \pm 0.005 \big)$ \\
\arrayrulecolor{gray}\cline{2-5}
 & \multirow{2}*{$\log_{10}M_{\rm sub}$} & \multirow{2}*{$8.91$} & pixelated & $8.71 \pm 0.05$ \\
 & & & refined & $8.90 \pm 0.01$ \\
 
\arrayrulecolor{black}\hline

\multirow{3}*{PS} & \multirow{3}*{$\big( \log_{10}\sigma^2_{\rm GRF}, \beta_{\rm GRF} \big)$} & \multirow{3}*{$\big( -3.11\pm0.15, 3.23\pm0.05 \big)$} & pixelated, ideal & $\big( -3.35\pm0.20, 3.40\pm0.15 \big)$ \\
 & & & pixelated, fiducial & $\big( -3.89\pm0.25, 4.15\pm0.19 \big)$ \\
 & & & pixelated, high-res & $\big( -3.49\pm0.15, 3.26\pm0.09\big)$ \\
 
\arrayrulecolor{black}\hline

\multirow{3}*{HM} & \multirow{2}*{$\big(a_m,\phi_m\big)$} & \multirow{2}*{$\big( 0.06, 82.50 \big)$} & pixelated & $\big( 0.024 \pm 0.002, 83.78 \pm 0.88 \big)$ \\
 & & & refined & $\big( 0.061 \pm 0.002, 83.15 \pm 0.39 \big)$ \\
 \arrayrulecolor{gray}\cline{2-5}
 & $m$ & $4$ & refined & $4.01 \pm 0.02$ \\
 
\arrayrulecolor{black}\hline
\end{tabular}
}
\end{table*}

==> Herculens - Wavelets in the potential with autodiff/table_notations.tex <==
\begin{table}[!h]
\caption{List of the main notations used in the paper.} \label{tab:notations}
\renewcommand{\arraystretch}{1.4}
\centering
{\small
\begin{tabular}{ll}

\hline
Notation & Definition \\
\hline\hline

\multicolumn{2}{l}{\textsl{Observation}} \\
\hline

\data & Imaging data \\
\datacovmatrix & Data covariance matrix \\
%$\sigma_\data$ & Data noise map $\equiv$ $\sqrt{ | {\rm diag} \left[ \datacovmatrix \right] | }$ \\

\hline
\multicolumn{2}{l}{\textsl{Model components}} \\
\hline

\model & Image model \\
\convop & Blurring operator \\
\lensingop & Lensing operator \\
\lenspot, \source, \lenslight & Lens potential, source light, lens light \\
%\lenspotmacro & Macro lensing potential \\
%\lenspotpert & Perturbations to the lensing potential \\

\hline
\multicolumn{2}{l}{\textsl{Model parametrization}} \\
\hline

\modelparam & Vector containing all model parameters \\
$\modelparam_{\lenspot}$, $\modelparam_{\source}$, $\modelparam_{\lenslight}$ & Parameters for analytical profiles $\tilde{\lenspot}$, $\tilde{\source}$, $\tilde{\lenslight}$ \\
\lenspotpix & Pixel values of the pixelated potential \\
$\lambda_{\rm\lenspotscalar,bl}$, $\lambda_{\rm\lenspotscalar,bl}$ & Regularization strengths for \lenspotpix \\
$\mat{W}_{\rm\lenspotscalar,bl}$, $\mat{W}_{\rm\lenspotscalar,bl}$ & Regularization weights for \lenspotpix \\

\hline
\multicolumn{2}{l}{\textsl{Optimization \& Inference}} \\
\hline

%\likelihoodsimple & Log-likelihood \\
%$\priorsimple_\lenspotscalar$, $\priorsimple_\sourcescalar$, $\priorsimple_\lenslightscalar$ & Log-priors (regularization terms) \\
\loss, \gradloss & Loss function and its gradient \\
\modelparamMAP & MAP solution  \\
$\mat{C}_\modelparam$ & Parameter covariance matrix \\
\hline
\end{tabular}
}
\end{table}


==> Herculens - Wavelets in the potential with autodiff/table_sim_input.tex <==
\begin{table}[!h]
\caption{Instrument settings and model assumptions used for generating HST/WFC3/F160W mock observations of EELs. The coordinates are oriented such as north is up and east is right. The orientation angle is east-of-north.} \label{app:tab:sim_params}
\renewcommand{\arraystretch}{1.2}
\centering
{\small
\begin{tabular}{lc}
\hline
\hline
\textbf{Observation} & \\
%\hline
Pixel size [arcsec] & 0.08 \\ 
%\hline
Exposure time [s] & $4\times2400 = 9600$ \\ 
%\hline
Zero-point [mag] & 25.9463 \\ 
%\hline
Sky brightness [mag/arcsec$^2$] & 22 \\ 
%\hline
Read noise [e$^-$] & 4 \\ 
%\hline
PSF (gaussian FWHM) [arcsec] & $0.3$ \\
%\hline
Noise & readout + shot noise \\
\hline
\hline
\textbf{Deflector, $\zd=0.3$} & \\
%\hline
\ \ \ Singular isothermal ellipsoid (SIE) & \\
\ \ \ \ \ \ Einstein radius, $\theta_{\rm E}$ [arcsec] & 1.6 \\
\ \ \ \ \ \ Ellipticity, $q_{\rm m}$ & 0.73 \\
\ \ \ \ \ \ Orientation, $\phi_{\rm m}$ & 82.5 \\
\ \ \ \ \ \ Position, ($x$, $y$) [arcsec] & $(0, 0)$ \\
\hline
\ \ \ External shear & \\
\ \ \ \ \ \ Strength, $\gamma_{\rm ext}$ & 0.032 \\
\ \ \ \ \ \ Orientation, $\phi_{\rm ext}$ & 144.2 \\
\hline
\ \ \ Sérsic (light) & \\
\ \ \ \ \ \ Ellipticity, $q_{\rm l}$ & $0.73\ (=q_{\rm m})$ \\
\ \ \ \ \ \ Orientation, $\phi_{\rm l}$ & $82.5\ (=\phi_{\rm m})$ \\
\ \ \ \ \ \ Half-light radius, $\theta_{\rm eff}$ & 2 \\
\ \ \ \ \ \ Sérsic index, $n_{\rm Sersic}$ & 2 \\
\ \ \ \ \ \ Position, ($x$, $y$) [arcsec] & $(0, 0)$ \\
\ \ \ \ \ \ Magnitude & 19 \\
\hline\hline
\textbf{Perturbations to the potential} & \\
%\hline
\ \ \ \textbf{LS}: Localized subhalo (SIS) & \\
\ \ \ \ \ \ Einstein radius, $\theta_{\rm E,halo}$ [arcsec] & 0.07 \\
\ \ \ \ \ \ Position, ($x$, $y$) [arcsec] & $(1.9, -0.4)$ \\
\hline
\ \ \ \textbf{PS}: Population of subhalos (GRF) & \\
\ \ \ \ \ \ Variance, $\sigma^2_{\rm GRF}$ & $10^{-3}$ \\
\ \ \ \ \ \ Slope, $\beta_{\rm GRF}$ & $4$ \\
\hline
\ \ \ \textbf{HM}: High-order moments (octupole) & \\
\ \ \ \ \ \ Strength, $a_4$ & $0.06$ \\
\ \ \ \ \ \ Orientation, $\phi_{\rm 4}$ & $82.5=\phi_{\rm m}$ \\
\hline\hline
\textbf{Source, $\zs=0.7$} & \\
%\hline
\ \ \ Sérsic & \\
\ \ \ \ \ \ Ellipticity, $q_{\rm l}$ & 0.82 \\
\ \ \ \ \ \ Orientation, $\phi_{\rm l}$ & 170.8 \\
\ \ \ \ \ \ Half-light radius, $\theta_{\rm eff}$ [arcsec] & 0.8 \\
\ \ \ \ \ \ Sérsic index, $n_{\rm Sersic}$ & 2 \\
\ \ \ \ \ \ Position ($x$, $y$) [arcsec] & $(0.4, 0.15)$ \\
\ \ \ \ \ \ Magnitude & 21 \\
\hline
\end{tabular}
}
\end{table}

